Chaotic and time-periodic edge states in square duct flow

We analyse the dynamics within the stability boundary between laminar and turbulent square duct flow with the aid of an edge-tracking algorithm. As for the circular pipe, the edge state turns out to be a chaotic attractor within the edge if the flow is not constrained to a symmetric subspace. The chaotic edge state dynamics is characterised by a sequence of alternating quiescent phases and regularly occurring bursting episodes. These latter reflect the different stages of the well-known streak-vortex interaction in near-wall turbulence: The edge states feature most of the time a single streak with a number of flanking quasi-streamwise vortices attached to one of the four surrounding walls. The initially straight streak undergoes the classical linear instability and eventually breaks in an intense bursting event due to the action of the quasi-streamwise vortices. At the same time, the vortices give rise to a new generation of low-speed streaks at one of the neighbouring walls, thereby causing the turbulent activity to `switch' from one wall to the other. When restricting the edge dynamics to a single or twofold mirror-symmetric subspace, on the other hand, the outlined bursting and wall-switching episodes become self-recurrent in time. These edge states thus represent the first periodic orbits found in the square duct. In contrast to the chaotic edge states in the non-symmetric case, the imposed symmetries enforce analogue bursting cycles to simultaneously appear at two parallel opposing walls in a mirror-symmetric configuration. Both localisation of the turbulent activity to one or two walls and wall switching are shown to be a common phenomenon in low Reynolds number duct turbulence. We therefore argue that the marginally turbulent trajectories transiently visit the identified edge states during these episodes, so that the edge states become actively involved in the turbulent dynamics.

==> Tikz_instructions.tex <==
%% --------------------------------------------------------------------------------------
%% dimensioning in figure
%% ------------------------

\usepackage{graphicx,tikz}
\usetikzlibrary{decorations,decorations.markings,decorations.text}
\usetikzlibrary{arrows.meta}

\pgfkeys{/pgf/decoration/.cd,
      distance/.initial=10pt
}  

\pgfdeclaredecoration{add dim}{final}{
\state{final}{% 
\pgfmathsetmacro{\dist}{5pt*\pgfkeysvalueof{/pgf/decoration/distance}/abs(\pgfkeysvalueof{/pgf/decoration/distance})}    
          \pgfpathmoveto{\pgfpoint{0pt}{0pt}}             
          \pgfpathlineto{\pgfpoint{0pt}{2*\dist}}   
          \pgfpathmoveto{\pgfpoint{\pgfdecoratedpathlength}{0pt}} 
          \pgfpathlineto{\pgfpoint{(\pgfdecoratedpathlength}{2*\dist}}     
          \pgfsetarrowsstart{latex}
          \pgfsetarrowsend{latex}
          \pgfpathmoveto{\pgfpoint{0pt}{\dist}}
          \pgfpathlineto{\pgfpoint{\pgfdecoratedpathlength}{\dist}} 
          \pgfusepath{stroke} 
          \pgfpathmoveto{\pgfpoint{0pt}{0pt}}
          \pgfpathlineto{\pgfpoint{\pgfdecoratedpathlength}{0pt}}
}}

\tikzset{dim/.style args={#1,#2}{decoration={add dim,distance=#2},
                decorate,
                postaction={decorate,decoration={text along path,
                								 text align={align=center},
                								 raise=#2,
                                                 text={#1}}}}}


%% --------------------------------------------------------------------------------------
%% Plot nice 3D arrows
%% ------------------------

\pgfkeys{
  /pgf/arrow keys/.cd,
  pitch/.code={%
    \pgfmathsetmacro\pgfarrowpitch{#1}
    \pgfmathsetmacro\pgfarrowsinpitch{abs(sin(\pgfarrowpitch))}
    \pgfmathsetmacro\pgfarrowcospitch{abs(cos(\pgfarrowpitch))}
  },
}

\pgfdeclarearrow{
  name = Cone,
  defaults = {       % inherit from Kite
    length     = +3.6pt +5.4,
    width'     = +0pt +0.5,
    line width = +0pt 1 1,
    pitch      = +0, % lie on screen
  },
  cache = false,     % no need cache
  setup code = {},   % so no need setup
  drawing code = {   % but still need math
    % draw the base
    \pgfmathsetmacro\pgfarrowhalfwidth{.5\pgfarrowwidth}
    \pgfmathsetmacro\pgfarrowhalfwidthsin{\pgfarrowhalfwidth*\pgfarrowsinpitch}
    \pgfpathellipse{\pgfpointorigin}{\pgfqpoint{\pgfarrowhalfwidthsin pt}{0pt}}{\pgfqpoint{0pt}{\pgfarrowhalfwidth pt}}
    \pgfusepath{fill}
    % test if the cone part visible
    \pgfmathsetmacro\pgfarrowlengthcos{\pgfarrowlength*\pgfarrowcospitch}
    \pgfmathparse{\pgfarrowlengthcos>\pgfarrowhalfwidthsin}
    \ifnum\pgfmathresult=1
      % it is visible, so draw
      \pgfmathsetmacro\pgfarrowlengthtemp{\pgfarrowhalfwidthsin*\pgfarrowhalfwidthsin/\pgfarrowlengthcos}
      \pgfmathsetmacro\pgfarrowwidthtemp{\pgfarrowhalfwidth/\pgfarrowlengthcos*sqrt(\pgfarrowlengthcos*\pgfarrowlengthcos-\pgfarrowhalfwidthsin*\pgfarrowhalfwidthsin)}
      \pgfpathmoveto{\pgfqpoint{\pgfarrowlengthcos pt}{0pt}}
      \pgfpathlineto{\pgfqpoint{\pgfarrowlengthtemp pt}{ \pgfarrowwidthtemp pt}}
      \pgfpathlineto{\pgfqpoint{\pgfarrowlengthtemp pt}{-\pgfarrowwidthtemp pt}}
      \pgfpathclose
      \pgfusepath{fill}
    \fi
    \pgfpathmoveto{\pgfpointorigin}
  }
}
